PCEvE: Part Contribution Evaluation Based Model Explanation for Human Figure Drawing Assessment and Beyond

For automatic human figure drawing (HFD) assessment tasks, such as diagnosing autism spectrum disorder (ASD) using HFD images, the clarity and explainability of a model decision are crucial. Existing pixel-level attribution-based explainable AI (XAI) approaches demand considerable effort from users to interpret the semantic information of a region in an image, which can be often time-consuming and impractical. To overcome this challenge, we propose a part contribution evaluation based model explanation (PCEvE) framework. On top of the part detection, we measure the Shapley Value of each individual part to evaluate the contribution to a model decision. Unlike existing attribution-based XAI approaches, the PCEvE provides a straightforward explanation of a model decision, i.e., a part contribution histogram. Furthermore, the PCEvE expands the scope of explanations beyond the conventional sample-level to include class-level and task-level insights, offering a richer, more comprehensive understanding of model behavior. We rigorously validate the PCEvE via extensive experiments on multiple HFD assessment datasets. Also, we sanity-check the proposed method with a set of controlled experiments. Additionally, we demonstrate the versatility and applicability of our method to other domains by applying it to a photo-realistic dataset, the Stanford Cars.

==> figure/fig_ASD-TD.tex <==
\begin{figure}[t]
\centering
% \mpage{0.48}{
\begin{minipage}[t]{0.48\textwidth}
\vtop{
\centering
\includegraphics[width=1.0\linewidth]{figure/img_files/results/class-level/asd-td/class-level-asd-td.pdf}

% After revision by Jinwoo
\caption{\textbf{The class-level PCEvE on the ASD Screening~\cite{jongmin2022autism} dataset.} We show the class-level part contribution histogram generated by the \method{}. 
%
The histogram shows that `face' contributes the most when the model recognizes ASD and TD samples.
%
The model tends to focus more on the `face' and less on `ear' and `hand' when recognizing TD samples on average, compared to when recognizing ASD samples.
}
\label{fig:class-level-ASD-TD}
}
\end{minipage}
% \mpage{0.48}{
\begin{minipage}[t]{0.48\textwidth}
\centering
\includegraphics[width=\linewidth]{figure/img_files/results/task-level/task-level-asd-td.pdf}
\\
\mpage{0.02}{\scriptsize(a)}
\hfill
% \mpage{0.20}{\scriptsize Face drawn by ASD children}
\mpage{0.22}{\centering \scriptsize ASD's face}
\hfill
\mpage{0.645}{
\includegraphics[width=0.74\linewidth]{figure/img_files/results/task-level/asd-samples.pdf}
}
\\
\mpage{0.02}{\scriptsize(b)}
\hfill
% \mpage{0.20}{\scriptsize Face drawn by TD children}
\mpage{0.21}{\centering \scriptsize TD's face}
\hfill
\mpage{0.645}{
\includegraphics[width=0.74\linewidth]{figure/img_files/results/task-level/td-samples.pdf}
}

% After revision by Jinwoo
\caption{\textbf{The task-level PCEvE on the ASD Screening~\cite{jongmin2022autism} dataset.} 
We show the task-level part contribution histogram generated by the \method{}. 
%
The histogram indicates that the model tends to focus on `face' to distinguish ASD and TD samples in the dataset.
%
We also visualize a few examples of `face' drawn by ASD children in (a) and drawn by TD children in (b).
%
We can see the distinct characteristics of drawings from ASD and TD children.
}
\label{fig:task-level-ASD-TD}
\end{minipage}
\end{figure}

==> figure/fig_class_level_ASD-TD-2.tex <==
\begin{figure}[t]
    \mpage{0.99}{
    \centering
    \small
    The 'ASD' class}
    \mpage{0.83}{
    \centering
    \includegraphics[width=\linewidth]{figure/img_files/results/class-level/asd-td/class-level-asd.png}
    }
    \hfill
    \mpage{0.145}{
    \centering
    \includegraphics[width=\linewidth]{figure/img_files/results/class-level/asd-td/class-level-asd-samples.png}
    }
    \vspace{-1em}
    \\
    \mpage{0.8}{(a)}
    \hfill
    \mpage{0.13}{(b)}

    \mpage{1.0}{}

    \mpage{0.99}{
    \centering
    \small
    The 'TD' class}
    \mpage{0.83}{
    \centering
    \includegraphics[width=\linewidth]{figure/img_files/results/class-level/asd-td/class-level-td.png}
    }
    \hfill
    \mpage{0.145}{
    \centering
    \includegraphics[width=\linewidth]{figure/img_files/results/class-level/asd-td/class-level-td-samples.png}
    }
    \vspace{-1em}
    \\
    \mpage{0.8}{(c)}
    \hfill
    \mpage{0.13}{(d)}

\caption{\textbf{Class-level PSV results on ASD-TD dataset.} We show class-level aggregating results for the PSV analysis on ASD-TD dataset.}
\label{fig:class-level-ASD-TD-2}
\end{figure}

==> figure/fig_switching_game.tex <==
\begin{figure}[t]
\centering
\footnotesize
% \includegraphics[width=\linewidth]{figure/img_files/discussion/switching-game/switching-game-asd-td.pdf}
% \\
\includegraphics[width=\linewidth]{figure/img_files/discussion/switching-game/switching-game-asd-td.pdf}
% \\
% \includegraphics[width=\linewidth]{figure/img_files/discussion/switching-game/switching-game-asd-td-3.pdf}
\\
(a) Swapping the `Face' part between an `ASD' sample and a `TD' sample
\\
\includegraphics[width=\linewidth]{figure/img_files/discussion/switching-game/switching-game-scat-3.pdf}
\\
(b) Swapping the `Hair' part between a `Male' sample and a `Female' sample
\\

% before revision by Jinwoo
% \caption{\textbf{Switching game.} We perform a `switching game' on the ASD Screening~\cite{jongmin2022autism} and SCAT datasets.
% In both (a) and (b), we observe reversal in the class prediction results when we swap the most important part identified through PCEvE analysis between the two samples. This indicates that PCEvE analysis can correctly identify the part that has the most influence on the model's prediction.
% }
% after revision by Jinwoo
\caption{\textbf{Part Switching Game Results.} 
We play a `part switching game' on the ASD Screening and SCAT datasets.
%
For each dataset, we pick two samples from two different classes and switch the most contributing part of each sample determined by the \method{} with each other.
%
Then we compare the model decisions with and without switching the parts.
%
In both (a) the ASD Screening and (b) the SCAT datasets (drawing gender classification), we observe the class prediction of the model reverts with part switching.
%
The results indicate that the \method{} can correctly identify the part contributing most to the model decision.
}
% In (a), when we swap the `Face' part between an `ASD' sample and a `TD' sample, both identified with their `Face' part being the most important, we observe a reversal in the class prediction results. `A' means the logit value of `ASD' class and `T' means the logit value of `TD' class.
% And in (b), when we swap the `Hair' part between a `Male' sample and a `Female' sample, both identified with their `Hair' part being the most important, we observe a reversal in the class prediction results. `M' means the logit value of `Male' class and `F' means the logit value of `Female' class.
\label{fig:switching-game}
\end{figure}

==> figure/fig_task_level_ASD-TD-2.tex <==
\begin{figure}[t]

\includegraphics[width=\linewidth]{figure/img_files/results/task-level/task-level-asd-td.png}

\caption{\textbf{Task-level PSV results on ASD-TD dataset.} We display task-level aggregating results for the PSV analysis on ASD-TD dataset. The 'Face' part is the most important for determining the sample's class to 'ASD' or 'TD'.}
\label{fig:task-level-ASD-TD-2}
\end{figure}

==> figure/fig_vits_class_level.tex <==
\begin{figure}[t]
\centering
\footnotesize
\mpage{0.485}{
\includegraphics[width=\linewidth]{figure/img_files/results/class-level/scat/vits-class-level-scat-drawing.pdf}
\\
(a) Part contribution histogram of the drawing gender classifier
}
\hfill
\mpage{0.485}{
\includegraphics[width=\linewidth]{figure/img_files/results/class-level/cars/vits-class-level-cars-cab.pdf}
\\
(b) Part contribution histogram of the car-type classifier
}

% Before revision by Jinwoo
% \caption{\textbf{The class-level PCEvE analysis using ViT-Small.}
% We show the class-level aggregating results for the PCEvE analysis on the SCAT and Stanford Cars~\cite{krause2013car} datasets using ViT~\cite{dosovitskiy2021vit} model. 
% We count the number of samples in which each part is identified as the most important part within a class and present this count in the form of frequencies.
% }

% After revision by Jinwoo
\caption{\textbf{The class-level part contribution evaluation based model explanation of the ViT-Small model.}
We show the class-level part contribution histograms generated by the class-level \method{} on the SCAT dataset (drawing gender classification) (a) and Stanford Cars datasets (b). 
\geo{We plot the result of the `Cab' class as a representative in the car-type classification task.}
%
Here we use the ViT-Small instead of EfficientNet-B1.
%
\geo{In (a) the drawing gender classification, the ViT-Small rely on the `Foot' part and the `Hair' part the most for the prediciton, just like the result using EfficientNet-B1 as shown in \figref{class-level-SCAT} (a). 
However, in (b) the car-type classification, the ViT-Small relies on the `Wheel' part the most for predicting 'Cab' samples, unlike the EfficientNet does in \figref{class-level-cars} (a).}
}
\label{fig:vit-small-results}
\end{figure}


==> table/part_inference_asd_addition.tex <==
\begin{table}[ht]
\centering
\footnotesize
\caption{\tb{Part inference results of the ASD-TD dataset.} 
We show the result of the part inference experiments on the ASD-TD dataset.
We evaluate the performance when we use (a) inputs consisting of each part only or (b) inputs excluding each part only to validate our framework.
The part with higher value in the class-level PSV result should correspond to (a) higher inference accuracy in the addition experiment and (b) lower inference accuracy in the deletion experiment.
We report the average top-1 accuracy (\%) of 5-fold cross-validation setting. The gray numbers on the left indicate the ranking in the class-level PSV results.
}
\vspace{-1mm}
(a) Addition
\\
\vspace{3mm}
\hfill
\mpage{0.45}{
The 'ASD' class
\\
\vspace{2mm}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
&Part & Acc. ($\uparrow$) \\ 
\midrule
&{\small Original image} & 98 \\
\cmidrule{2-3}
{\textcolor{gray}1} & Face & 100 \\
{\textcolor{gray}2} & Eye & 100 \\
{\textcolor{gray}3} & Ear & 98 \\
{\textcolor{gray}4} & Hand & 98 \\
{\textcolor{gray}5} & Foot & 94 \\
{\textcolor{gray}6} & Mouth & 96 \\
{\textcolor{gray}6} & Nose & 96 \\
\bottomrule
\end{tabular}
}
}
\mpage{0.45}{
The 'TD' class
\\
\vspace{2mm}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
&Part & Acc. ($\uparrow$) \\ 
\midrule
&{\small Original image} & 98 \\
\cmidrule{2-3}
{\textcolor{gray}1} & Face & 88 \\
{\textcolor{gray}2} & Mouth & 72 \\
{\textcolor{gray}3} & Foot & 74 \\
{\textcolor{gray}4} & Eye & 60 \\
{\textcolor{gray}4} & Nose & 70 \\
{\textcolor{gray}6} & Ear & 70 \\
{\textcolor{gray}6} & Hand & 76 \\
\bottomrule
\end{tabular}
}
}
\hfill
\\
\vspace{4mm}
(b) Deletion
\\
\vspace{3mm}
\hfill
\mpage{0.45}{
The 'ASD' class
\\
\vspace{2mm}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
&Part & Acc. ($\uparrow$) \\ 
\midrule
&{\small Original image} & 98 \\
\cmidrule{2-3}
{\textcolor{gray}1} & Face & 98 \\
{\textcolor{gray}2} & Eye & 98 \\
{\textcolor{gray}3} & Ear & 98 \\
{\textcolor{gray}4} & Hand & 96 \\
{\textcolor{gray}5} & Foot & 98 \\
{\textcolor{gray}6} & Mouth & 98 \\
{\textcolor{gray}6} & Nose & 98 \\
\bottomrule
\end{tabular}
}
}
\mpage{0.45}{
The 'TD' class
\\
\vspace{2mm}
\resizebox{.9\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
&Part & Acc. ($\uparrow$) \\ 
\midrule
&{\small Original image} & 98 \\
\cmidrule{2-3}
{\textcolor{gray}1} & Face & 74 \\
{\textcolor{gray}2} & Mouth & 94 \\
{\textcolor{gray}3} & Foot & 90 \\
{\textcolor{gray}4} & Eye & 98 \\
{\textcolor{gray}4} & Nose & 100 \\
{\textcolor{gray}6} & Ear & 92 \\
{\textcolor{gray}6} & Hand & 98 \\
\bottomrule
\end{tabular}
}
}
\hfill

\label{tab:model_acc}
\end{table}
